I know what leaked in your pocket: uncovering privacy leaks on Android Apps with Static Taint Analysis

Android applications may leak privacy data carelessly or maliciously. In this work we perform inter-component data-flow analysis to detect privacy leaks between components of Android applications. Unlike all current approaches, our tool, called IccTA, propagates the context between the components, which improves the precision of the analysis. IccTA outperforms all other available tools by reaching a precision of 95.0% and a recall of 82.6% on DroidBench. Our approach detects 147 inter-component based privacy leaks in 14 applications in a set of 3000 real-world applications with a precision of 88.4%. With the help of ApkCombiner, our approach is able to detect inter-app based privacy leaks.

==> figures/android-discontinuities.tex <==

\begin{tikzpicture}
\tikzstyle{nodeS} = [draw, minimum width=2cm, minimum height=.6cm]
\tikzstyle{emptyS} = [inner sep=0cm, outer sep=0cm]

\path (0,0) node {}
++(0, -.5cm)node[nodeS] (startA) {startActivity}
++(2.5cm, .5cm) node[nodeS] (onC) {onCreate}
+ (0,0) node[nodeS, dashed, minimum width=2.1cm, minimum height = .7cm] (onC2) {}
+(0,-1.6cm) node [draw, circle, outer sep = 0cm, inner sep = .0cm, double, text width=1.2cm, text centered] (AThread) {Android\\ System}
++(2.5cm, -.5cm) node[nodeS, dashed] (onS) {onStart}
++(0, -2.5cm) node[nodeS, densely dotted] (onCl) {onClick}
++(-4.5cm, 0) node[nodeS, densely dotted] (clEv) {Button Click Event}

++(-1.5cm,-.6cm) node[emptyS] (iccL) {}
++(1cm,0) node[emptyS, label=right:ICC \tiny] (iccR) {}
++(1.4cm,0) node[emptyS] (lcL) {}
++(1cm,0) node[emptyS, label=right:Lifecycle \tiny] (lcR) {}
++(1.9cm,0) node[emptyS] (cbL) {}
++(1cm,0) node[emptyS, label=right:Callback \tiny] (cbR) {}

+(0,-.6cm) {} %% space between figure and caption. Should NOT bet necessary, but depends on the template.
;

\draw[-latex] (startA) to[out=-50,in=180,distance=.8cm] (AThread);
\draw[-latex] (AThread) to[out=30,in=-40] (onC);

\draw[-latex, dashed] (onC2) to[out=-160,in=160,distance=.4cm] (AThread);
\draw[-latex, dashed] (AThread) to[out=0,in=-90,distance=.8cm] (onS);

\draw[-latex, densely dotted] (clEv) to[out=90,in=-160] (AThread);
\draw[-latex, densely dotted] (AThread) to[out=-15,in=90] (onCl);

%% legend
\draw[-latex] (iccL) -- (iccR);
\draw[-latex, dashed] (lcL) -- (lcR);
\draw[-latex, densely dotted] (cbL) -- (cbR);
\end{tikzpicture}


==> pie-macros.tex <==
\definecolor{rosso}{RGB}{220,57,18}
\definecolor{giallo}{RGB}{255,153,0}
\definecolor{blu}{RGB}{102,140,217}
\definecolor{verde}{RGB}{16,150,24}
\definecolor{viola}{RGB}{153,0,153}

\makeatletter

\tikzstyle{chart}=[
    legend label/.style={font={\scriptsize},anchor=west,align=left},
    legend box/.style={rectangle, draw, minimum size=5pt},
    axis/.style={black,semithick,->},
    axis label/.style={anchor=east,font={\tiny}},
]

\tikzstyle{bar chart}=[
    chart,
    bar width/.code={
        \pgfmathparse{##1/2}
        \global\let\bar@w\pgfmathresult
    },
    bar/.style={very thick, draw=white},
    bar label/.style={font={\bf\small},anchor=north},
    bar value/.style={font={\footnotesize}},
    bar width=.75,
]

\tikzstyle{pie chart}=[
    chart,
    slice/.style={line cap=round, line join=round, very thick,draw=white},
    pie title/.style={font={\bf}},
    slice type/.style 2 args={
        ##1/.style={fill=##2},
        values of ##1/.style={}
    }
]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}


\newcommand{\pie}[4][]{
    \begin{scope}[#1]
    \pgfmathsetmacro{\curA}{90}
    \pgfmathsetmacro{\r}{1}
    \def\c{(0,0)}
    \node[pie title] at (90:1.3) {#2};
    \foreach \v/\s/\p in #4{ % don't put #3 into brackets otherwise it will not work with list generated programatically
        \pgfmathsetmacro{\deltaA}{\v/#3*360}
        \pgfmathsetmacro{\nextA}{\curA + \deltaA}
        \pgfmathsetmacro{\midA}{(\curA+\nextA)/2}
        \pgfmathsetmacro{\percentage}{(\v/#3) * 100}

        \path[slice, fill=\s, draw=black, postaction={pattern=\p}] \c
            -- +(\curA:\r)
            arc (\curA:\nextA:\r)
            -- cycle;
        \pgfmathsetmacro{\d}{max((\deltaA * -(.5/50) + 1.15) , .7)}

        \begin{pgfonlayer}{foreground}
        \path \c -- node[pos=\d,pie values]{\footnotesize $\num[round-mode=places, round-precision=2]{\percentage}\%$} +(\midA:\r);
        \end{pgfonlayer}

        \global\let\curA\nextA
    }
    \end{scope}
}

\newcommand{\legend}[2][]{
    \begin{scope}[#1]
    \path
        \foreach \n/\s/\p in #2
            {
                  ++(0,-15pt) node[\s,legend box, pattern=\p, draw=black] {} +(5pt,0) node[legend label, text width=1.6cm] {\n}
            }
    ;
    \end{scope}
}

\newcommand{\testp}[3][]{

\pgfplotstableread[col sep=comma, ignore chars={"}]{#3}{\firsttable}   
\pgfplotstablegetrowsof{#3}
\pgfmathsetmacro{\rows}{\pgfplotsretval-1}  

\global\def\myresult{}
\global\def\mylegend{}
\gdef\mycount{0.0}
\gdef\co{55.0}
\pgfmathparse{(\co - 10) / \rows}
\xdef\step{\pgfmathresult}
\foreach \i in {0,...,\rows}{%
  \pgfplotstablegetelem{\i}{[index] 0}\of{\firsttable} 
  \let\xA\pgfplotsretval 
  \pgfplotstablegetelem{\i}{[index] 1}\of{\firsttable} 
  \let\yA\pgfplotsretval     
 
  \def\bcolor{black!\co} 
  \xdef\myresult{\myresult\ifx\myresult\empty\else,\fi\yA/\bcolor/}
  \xdef\mylegend{\mylegend\ifx\mylegend\empty\else,\fi\xA\ (\yA)/\bcolor/}
  
  \pgfmathparse{\mycount + \yA}
  \xdef\mycount{\pgfmathresult}
  \pgfmathparse{\co - \step}
  \xdef\co{\pgfmathresult}
}
\pie{#2}{\mycount}{ \myresult}
\legend[shift={(1.2cm,1.4cm)}]{\mylegend} 

}


